Abstract Compilation for Verification of Numerical Accuracy Properties

Verification of numerical accuracy properties in modern software remains an important and challenging task. This paper describes an original framework combining different solutions for numerical accuracy. First, we extend an existing runtime verification tool called E-ACSL with rational numbers to monitor accuracy properties at runtime. Second, we present an abstract compiler, FLDCompiler, that performs a source-to-source transformation such that the execution of the resulting program, called an abstract execution, is an abstract interpretation of the initial program. Third, we propose an instrumentation library FLDLib that formally propagates accuracy properties along an abstract execution. While each of these solutions has its own interest, we emphasize the benefits of their combination for an industrial setting. Initial experiments show that the proposed technique can efficiently and soundly analyze the accuracy of industrial programs by restricting the analysis on thin numerical scenarios.

==> multi-executions.tex <==
\commentJS{This section should disappear. Don't know yet whether its contents
will be put somewhere.}

E-ACSL integrates the formal properties to validate into the executable code.
This section considers the properties verifying that two (or more) executions
with different semantics are close enough. The accuracy
analyses~\cite{} \TODO{BIB} typically compare an execution where all
floating-point computations are ideal to an execution where the floating-point
computations follow the IEEE-754~\cite{} \TODO{BIB} standard.

An extension of E-ACSL could manage the inference of the accuracy properties by
replacing every floating-point value by a pair containing a conservative
interval for the ideal value and the original IEEE-754 value in the spirit of
FpDebug. But in case of unstable branches~\cite{} \TODO{BIB}, both computations
can take different execution flows as in the example

\lstset{language=C, keywordstyle=\bfseries\color{black},commentstyle=\color{gray}, showlines=true, moredelim=**[is][\color{gray}]{@}{@}, mathescape, basicstyle=\footnotesize}
\begin{lstlisting}
float x = 2.0 - 1e-15;
if (x < 2.0) res = 1+x; else res = 4-x;
\end{lstlisting}
The ideal computation executes the instruction {\texttt res = 1+x;} and the
IEEE-754 computation executes the instruction {\texttt res=4-x;} since the
closest floating point of {\texttt 2.0 - 1e-15} is {\texttt 2.0}.

The extension of E-ACSL we consider for the accuracy analysis has to provide
a sound execution covering both executions. We provide a way to do this on
a subset of the C language with an additional Frama-C plugin fld_compiler and an
instrumentation library like fldlib as despicted on the figure below.

The subset just offers the guarantee that the IEEE-754 execution flow will
eventually synchronize with the ideal execution flow.

